Sparx: Distributed Outlier Detection at Scale

There is no shortage of outlier detection (OD) algorithms in the literature, yet a vast body of them are designed for a single machine. With the increasing reality of already cloud-resident datasets comes the need for distributed OD techniques. This area, however, is not only understudied but also short of public-domain implementations for practical use. This paper aims to fill this gap: We design Sparx, a data-parallel OD algorithm suitable for shared-nothing infrastructures, which we specifically implement in Apache Spark. Through extensive experiments on three real-world datasets, with several billions of points and millions of features, we show that existing open-source solutions fail to scale up; either by large number of points or high dimensionality, whereas Sparx yields scalable and effective performance. To facilitate practical use of OD on modern-scale datasets, we open-source Sparx under the Apache license at https://tinyurl.com/sparx2022.

==> TABLE/datasets.tex <==


\begin{table}[!ht]
\caption{Datasets used for evaluation.
Shown in parentheses are the number of attributes.
 %In each dataset, the training set consists exclusively of inlier graphs, whereas the test set is polluted by outlier graphs which are $\sim 5\%$ of the inliers in number. Details of each dataset are provided in Section~\ref{sec:appendix}.
} 
\vspace{-0.15in}
\centering
\footnotesize{
\begin{tabular}{l|c|c|r|r}
	\toprule
	\rule{0pt}{2.5ex}\textbf{Name} & \textbf{Avg \#nodes} & \textbf{Type}  & $|$\textbf{Train}$|$ & $|$\textbf{Test}$|$ \\ \midrule
	\rule{0pt}{2.5ex}\textsc{Mixhop}  &         100          &    Labeled     &         532          &         493         \\
	\textsc{Proteins}                 &        39.06         &    Labeled     &         358          &         333         \\
	\textsc{Tox21}                    &        18.09         &    Labeled     &         472          &         503         \\
	\textsc{Collab}                   &        74.49         &    Labeled     &         395          &         397         \\
	\textsc{IMDB}                     &        19.77         &    Labeled     &         270          &         240         \\
	\textsc{NCI1}                     &        29.87         &    Labeled     &         1014         &        1096         \\
	\textsc{Mutagen}                  &        30.32         &    Labeled     &         1189         &        1274         \\
	\textsc{Reddit}                   &        23.93         &    Labeled     &         2418         &        2594         \\
	\textsc{DD}                       &        284.32        &    Labeled     &         375          &         336         \\
	\textsc{AIDS-L}                   &        15.69         &    Labeled     &         202          &         206         \\
	\textsc{DHFR-L}                   &        42.43         &    Labeled     &         154          &         147         \\ \hline
	\rule{0pt}{2.5ex}\textsc{BZR}     &        35.75         & Attributed (3) &         170          &         154         \\
	\textsc{COX2}                     &        41.22         & Attributed (3) &         195          &         176         \\
	\textsc{AIDS-A}                   &        15.69         & Attributed (4) &         202          &         206         \\
	\textsc{DHFR-A}                   &        42.43         & Attributed (3) &         154          &         147         \\ \bottomrule
\end{tabular}
}
\vspace{-0.15in}
	\label{table:data} 
\end{table}

==> TABLE/horserace.tex <==



\begin{table*}[!ht]
\caption[Comparison of anomaly detection performance of \method against baselines.]{Comparison of anomaly-detection performance of \method against baselines. For all baselines, we run the experiment over a grid of hyperparameter choices\footnotemark~and report the average and standard deviation of the ROC-AUC scores. As \method employs (unsupervised) model selection, it only outputs \underline{\bf one} ranking, and we simply report its ROC-AUC.} 
\centering
	\vspace{-0.15in}	
	\scalebox{0.9}{
\begin{tabular}{l|c|c|c|c|c|c|c|c||c}
	\toprule
	\multicolumn{1}{c|}{Dataset}     &         \pk-LOF          &        \pk-OCSVM         &         \wl-LOF          &        \wl-OCSVM         &       \gtovec-LOF        &      \gtovec-OCSVM       &         DOMINANT         &          OCGNN           &               GLAM                \\ \midrule
	\rule{0pt}{2.5ex}\textsc{Mixhop} &     0.67 $\pm$ 0.17      &     0.69 $\pm$ 0.14      &     0.72 $\pm$ 0.09      &     0.57 $\pm$ 0.01      &     0.67 $\pm$ 0.08      &     0.51 $\pm$ 0.03      & \textbf{1.00 $\pm$ 0.00} &            -             &               0.99                \\
	\textsc{Proteins}                &     0.68 $\pm$ 0.12      &     0.67 $\pm$ 0.09      &     0.72 $\pm$ 0.05      &     0.78 $\pm$ 0.03      &     0.47 $\pm$ 0.05      &     0.46 $\pm$ 0.09      &     0.48 $\pm$ 0.23      &     0.75 $\pm$ 0.34      &           \textbf{0.82}           \\
	\textsc{Tox21}                   &     0.53 $\pm$ 0.05      &     0.57 $\pm$ 0.04      &     0.65 $\pm$ 0.05      &     0.66 $\pm$ 0.02      &     0.47 $\pm$ 0.06      &     0.47 $\pm$ 0.06      &     0.53 $\pm$ 0.02      &     0.52 $\pm$ 0.05      &           \textbf{0.70}           \\
	\textsc{Collab}                  &     0.73 $\pm$ 0.05      &     0.78 $\pm$ 0.02      &     0.81 $\pm$ 0.06      &     0.84 $\pm$ 0.00      &     0.54 $\pm$ 0.18      &     0.75 $\pm$ 0.03      &     0.85 $\pm$ 0.02      &     0.58 $\pm$ 0.22      &           \textbf{0.87}           \\
	\textsc{IMDB}                    &     0.61 $\pm$ 0.09      &     0.68 $\pm$ 0.06      &     0.65 $\pm$ 0.04      &     0.63 $\pm$ 0.03      &     0.45 $\pm$ 0.09      &     0.35 $\pm$ 0.04      &     0.62 $\pm$ 0.01      &     0.51 $\pm$ 0.05      &           \textbf{0.70}           \\
	\textsc{NCI1}                    &     0.64 $\pm$ 0.06      &     0.45 $\pm$ 0.07      & \textbf{0.73 $\pm$ 0.04} &     0.60 $\pm$ 0.08      &     0.48 $\pm$ 0.10      &     0.33 $\pm$ 0.11      &     0.49 $\pm$ 0.12      &     0.45 $\pm$ 0.16      &               0.59                \\
	\textsc{Mutagen}                 &     0.57 $\pm$ 0.05      &     0.53 $\pm$ 0.02      &     0.56 $\pm$ 0.03      &     0.52 $\pm$ 0.03      & \textbf{0.64 $\pm$ 0.04} &     0.57 $\pm$ 0.05      &     0.59 $\pm$ 0.07      &     0.49 $\pm$ 0.06      &               0.59                \\
	\textsc{Reddit}                  &     0.45 $\pm$ 0.06      &     0.75 $\pm$ 0.02      &     0.54 $\pm$ 0.14      & \textbf{0.83 $\pm$ 0.01} &     0.43 $\pm$ 0.07      &     0.58 $\pm$ 0.04      &            -             &            -             &               0.76                \\
	\textsc{DD}                      &     0.83 $\pm$ 0.06      &     0.76 $\pm$ 0.04      & \textbf{0.92 $\pm$ 0.01} &     0.91 $\pm$ 0.01      &     0.31 $\pm$ 0.03      &     0.46 $\pm$ 0.03      &            -             &     0.60 $\pm$ 0.06      &               0.84                \\
	\textsc{AIDS-L}                  &     0.77 $\pm$ 0.11      &     0.73 $\pm$ 0.10      & \textbf{0.95 $\pm$ 0.04} &     0.94 $\pm$ 0.07      &     0.30 $\pm$ 0.16      &     0.12 $\pm$ 0.12      &     0.68 $\pm$ 0.04      &     0.42 $\pm$ 0.14      &               0.91                \\
	\textsc{DHFR-L}                  &     0.64 $\pm$ 0.07      &     0.74 $\pm$ 0.05      &     0.77 $\pm$ 0.07      &     0.81 $\pm$ 0.05      &     0.62 $\pm$ 0.12      &     0.40 $\pm$ 0.08      &     0.36 $\pm$ 0.07      &     0.37 $\pm$ 0.14      &           \textbf{0.83}           \\
	\textsc{BZR}                     & \textbf{0.69 $\pm$ 0.11} &     0.58 $\pm$ 0.06      &            -             &            -             &            -             &            -             &     0.37 $\pm$ 0.01      &     0.55 $\pm$ 0.07      &               0.55                \\
	\textsc{COX2}                    &     0.70 $\pm$ 0.05      &     0.55 $\pm$ 0.10      &            -             &            -             &            -             &            -             &     0.42 $\pm$ 0.02      &     0.56 $\pm$ 0.13      &           \textbf{0.71}           \\
	\textsc{AIDS-A}                  &     0.53 $\pm$ 0.12      &     0.84 $\pm$ 0.04      &            -             &            -             &            -             &            -             &     0.05 $\pm$ 0.00      &     0.43 $\pm$ 0.11      &           \textbf{0.94}           \\
	\textsc{DHFR-A}                  &     0.70 $\pm$ 0.06      &     0.62 $\pm$ 0.03      &            -             &            -             &            -             &            -             &     0.43 $\pm$ 0.00      &     0.58 $\pm$ 0.06      &           \textbf{0.82}           \\ \midrule
	\textit{avg (labeled)}           & \textit{0.65 $\pm$ 0.11} & \textit{0.67 $\pm$ 0.11} & \textit{0.73 $\pm$ 0.13} & \textit{0.74 $\pm$ 0.14} & \textit{0.49 $\pm$ 0.13} & \textit{0.47 $\pm$ 0.15} & \textit{0.62 $\pm$ 0.20} & \textit{0.52 $\pm$ 0.11} & \textit{\textbf{0.78 $\pm$ 0.13}} \\
	\textit{avg (all)}               & \textit{0.65 $\pm$ 0.10} & \textit{0.66 $\pm$ 0.11} &            -             &            -             &            -             &            -             & \textit{0.53 $\pm$ 0.24} & \textit{0.52 $\pm$ 0.10} & \textit{\textbf{0.77 $\pm$ 0.13}} \\ \bottomrule
\end{tabular}
	}
	\vspace{-0.1in}
	\label{table:horserace} 
\end{table*}

==> TABLE/tabcompare.tex <==



\begin{table*}
	\caption{Comparison of related work in terms of desired properties for graph-level anomaly detection. Also see Sec. \ref{sec:related}.}
	\label{tab:related}
	\vspace{-0.15in}	
	\scalebox{0.9}{
		\begin{tabular}{l|c|ccc|ccc|ccc|c}
			\toprule
			& 
			\cite{chalapathy2019learning,journals/corr/abs-2009-11732} &
			% % % % % % % % % % % % % % % %
			\cite{deepwalk2014,conf/nips/HamiltonYL17,conf/cikm/0003DYJW020,conf/kdd/YuCAZCW18} & %DeepWalk, GraphSage, GAL, Netwalk
			\cite{ocgnn20,conf/sdm/DingLBL19} &  % OCGNN, % DOMINANT
			\cite{KumagaiIF20} &  
			% % % % % % % % % % % % % % % % %
			\cite{conf/kdd/NobleC03}  & % Subdue
			\cite{conf/kdd/ManzoorMA16} &     % StreamSpot 
			\cite{conf/kdd/EswaranFGM18} & % SpotLight
			
			% % % % % % % % % % % % % % % % % % % % % %
			\cite{pmlr-v48-niepert16,conf/iclr/XuHLJ19} & %GIN, PATCHY-SAN
			\cite{neumann2016propagation} &  %  PK
			\cite{NarayananCVCLJ17,shervashidze2011weisfeiler} & % graph2vec, WL kernel
			%	auto-encoder &  
			this  \\	
			\textbf{Desired Properties}  & point-cloud 	& 	\multicolumn{3}{c|}{node-level} & \multicolumn{3}{c|}{traditional}& \multicolumn{3}{c|}{graph embedding} & paper \\
			\midrule
			%end-to-end anomaly detection (vs. two-stage) & \cmark& & \cmark	&	 \cmark&		\cmark&	\cmark	&\cmark	& &		 & &  \cmark\\\hline
			end-to-end anomaly detection  & \cmark& & \cmark	&	 \cmark&		&		&	& &		 & &  \cmark\\\hline
			unsupervised (vs. (semi-)supervised)		&  \cmark&	\cmark	& \cmark	&	&	\cmark & \cmark& \cmark&	&  \cmark	& \cmark&	\cmark \\\hline
			graph-structured data (vs. point-cloud) 	&  	  & \cmark & \cmark	&	 \cmark&\cmark&	\cmark	&\cmark &	\cmark &\cmark &\cmark &	  \cmark\\\hline
			graph-level detection (vs. node/edge-level) &  	  	& &		&	& \cmark&	\cmark	&\cmark&\cmark	& \cmark &  \cmark&	 \cmark\\\hline
			graph embedding 			& 	& & 	&	&  &	 \cmark& \cmark	&\cmark &	\cmark	& \cmark&\cmark	\\\hline
			handle labeled nodes 							& 	& \cmark &	 \cmark &	 \cmark &\cmark&	\cmark & &	\cmark& \cmark &\cmark&	 	 \cmark\\\hline
			handle multi-attributed nodes						&  			&\cmark & \cmark& 	 \cmark&& & &	\cmark&	\cmark &	    	& 	 \cmark\\\hline
			handle  weighted edges	&  & \cmark	& \cmark	&\cmark	& 	& & \cmark	&\cmark	&\cmark	&	& 	\cmark \\\hline
			unsupervised model selection					&  &	&	&	&	& & 	& 		& 	&	&\cmark \\	
			\bottomrule
		\end{tabular}
	}
\end{table*}


